Power Modeling for Virtual Reality Video Playback Applications

This paper proposes a method to evaluate and model the power consumption of modern virtual reality playback and streaming applications on smartphones. Due to the high computational complexity of the virtual reality processing toolchain, the corresponding power consumption is very high, which reduces operating times of battery-powered devices. To tackle this problem, we analyze the power consumption in detail by performing power measurements. Furthermore, we construct a model to estimate the true power consumption with a mean error of less than 3.5%. The model can be used to save power at critical battery levels by changing the streaming video parameters. Particularly, the results show that the power consumption is significantly reduced by decreasing the input video resolution.

==> gfx/bars_max_power_contrib_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{15.40}{15.40}\selectfont\strut}%
\psfrag{020}[tc][tc]{\matlabtextA Maximum Power Contribution}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{14.00}{14.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.2$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.4$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.6$}%
\psfrag{004}[ct][ct]{\matlabtextB $0.8$}%
\psfrag{005}[ct][ct]{\matlabtextB $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $1$}%
\psfrag{007}[rc][rc]{\matlabtextB $2$}%
\psfrag{008}[rc][rc]{\matlabtextB $3$}%
\psfrag{009}[rc][rc]{\matlabtextB $4$}%
\psfrag{010}[rc][rc]{\matlabtextB $5$}%
\psfrag{011}[rc][rc]{\matlabtextB $6$}%
\psfrag{012}[rc][rc]{\matlabtextB $7$}%
\psfrag{013}[rc][rc]{\matlabtextB $8$}%
\psfrag{014}[rc][rc]{\matlabtextB $9$}%
\psfrag{015}[rc][rc]{\matlabtextB $10$}%
\psfrag{016}[rc][rc]{\matlabtextB $11$}%
\psfrag{017}[rc][rc]{\matlabtextB $12$}%
\psfrag{018}[rc][rc]{\matlabtextB $13$}%
\psfrag{019}[rc][rc]{\matlabtextB $14$}%
%
%% </ytick>

==> gfx/bars_power03_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{12.60}{12.60}\selectfont\strut}%
\psfrag{000000000000000000000000}[cl][cl]{\matlabtextA data1aaaaaaaaaaaaaaaa}%
\psfrag{001}[cl][cl]{\matlabtextA }%
\psfrag{002}[cl][cl]{\matlabtextA }%
\psfrag{003}[cl][cl]{\matlabtextA }%
\psfrag{004}[cl][cl]{\matlabtextA }%
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{15.40}{15.40}\selectfont\strut}%
\psfrag{017}[tc][tc]{\matlabtextB Power [W]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextC{\color[rgb]{0.150,0.150,0.150}\fontsize{14.00}{14.00}\selectfont\strut}%
\psfrag{005}[ct][ct]{\matlabtextC $0$}%
\psfrag{006}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{007}[ct][ct]{\matlabtextC $1$}%
\psfrag{008}[ct][ct]{\matlabtextC $1.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextC $1$}%
\psfrag{010}[rc][rc]{\matlabtextC $2$}%
\psfrag{011}[rc][rc]{\matlabtextC $4$}%
\psfrag{012}[rc][rc]{\matlabtextC $5$}%
\psfrag{013}[rc][rc]{\matlabtextC $7$}%
\psfrag{014}[rc][rc]{\matlabtextC $8$}%
\psfrag{015}[rc][rc]{\matlabtextC $10$}%
\psfrag{016}[rc][rc]{\matlabtextC $11$}%
%
%% </ytick>

==> gfx/maxContrib_for_Model2_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{15.40}{15.40}\selectfont\strut}%
\psfrag{017}[tc][tc]{\matlabtextA Power}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{14.00}{14.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.2$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.4$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.6$}%
\psfrag{004}[ct][ct]{\matlabtextB $0.8$}%
\psfrag{005}[ct][ct]{\matlabtextB $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $1$}%
\psfrag{007}[rc][rc]{\matlabtextB $2$}%
\psfrag{008}[rc][rc]{\matlabtextB $3$}%
\psfrag{009}[rc][rc]{\matlabtextB $4$}%
\psfrag{010}[rc][rc]{\matlabtextB $5$}%
\psfrag{011}[rc][rc]{\matlabtextB $6$}%
\psfrag{012}[rc][rc]{\matlabtextB $7$}%
\psfrag{013}[rc][rc]{\matlabtextB $8$}%
\psfrag{014}[rc][rc]{\matlabtextB $9$}%
\psfrag{015}[rc][rc]{\matlabtextB $10$}%
\psfrag{016}[rc][rc]{\matlabtextB $11$}%
%
%% </ytick>

==> gfx/power_VR03_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{15.40}{15.40}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextA Power [W]}%
\psfrag{013}[bc][bc]{\matlabtextA Time [s]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{14.00}{14.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $2$}%
\psfrag{002}[ct][ct]{\matlabtextB $4$}%
\psfrag{003}[ct][ct]{\matlabtextB $6$}%
\psfrag{004}[ct][ct]{\matlabtextB $8$}%
\psfrag{005}[ct][ct]{\matlabtextB $10$}%
\psfrag{006}[ct][ct]{\matlabtextB $12$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $2$}%
\psfrag{009}[rc][rc]{\matlabtextB $4$}%
\psfrag{010}[rc][rc]{\matlabtextB $6$}%
\psfrag{011}[rc][rc]{\matlabtextB $8$}%
%
%% </ytick>

==> gfx/power_VR_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.7.0devb04
% Version Date: 30-May-2013
% Author: Zebb Prime
%
\providecommand\matlabfragNegTickNoWidth{\makebox[0pt][r]{\ensuremath{-}}}%
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{15.40}{15.40}\selectfont\strut}%
\psfrag{011}[tc][tc]{\matlabtextA Time [s]}%
\psfrag{012}[bc][bc]{\matlabtextA Power [mW]}%
%
%% </text>
%
%% <xtick>
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{14.00}{14.00}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $2$}%
\psfrag{002}[ct][ct]{\matlabtextB $4$}%
\psfrag{003}[ct][ct]{\matlabtextB $6$}%
\psfrag{004}[ct][ct]{\matlabtextB $8$}%
\psfrag{005}[ct][ct]{\matlabtextB $10$}%
\psfrag{006}[ct][ct]{\matlabtextB $12$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $2$}%
\psfrag{009}[rc][rc]{\matlabtextB $4$}%
\psfrag{010}[rc][rc]{\matlabtextB $6$}%
%
%% </ytick>
